Constrained Posterior Sampling: Time Series Generation with Hard Constraints

Generating realistic time series samples is crucial for stress-testing models and protecting user privacy by using synthetic data. In engineering and safety-critical applications, these samples must meet certain hard constraints that are domain-specific or naturally imposed by physics or nature. Consider, for example, generating electricity demand patterns with constraints on peak demand times. This can be used to stress-test the functioning of power grids during adverse weather conditions. Existing approaches for generating constrained time series are either not scalable or degrade sample quality. To address these challenges, we introduce Constrained Posterior Sampling (CPS), a diffusion-based sampling algorithm that aims to project the posterior mean estimate into the constraint set after each denoising update. Notably, CPS scales to a large number of constraints ($\sim100$) without requiring additional training. We provide theoretical justifications highlighting the impact of our projection step on sampling. Empirically, CPS outperforms state-of-the-art methods in sample quality and similarity to real time series by around 70\% and 22\%, respectively, on real-world stocks, traffic, and air quality datasets.

==> figures_latex/cps_prodigy.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.95\textwidth]{figures/cps_prodigy.pdf}
    \vskip -0.15in
    \caption{\textbf{Qualitative comparison between PRODIGY \citep{sharma2024diffuse} and \projectabbr\ on the real-world datasets used in our experiments.}}
    
    \label{fig:cps_prodigy}
\end{center}
\vskip -0.2in
\end{figure*}

==> figures_latex/review_qualitative.tex <==
\begin{figure*}[!hbt]
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/review_plot.pdf}
    \vspace{-0.5cm}
    \caption{\rebuttal{\textbf{\projectabbr\ provides high-fidelity synthetic time series samples that adhere to the required constraints and track the real time series data.} Here, we show multiple generations (10) of the same qualitative examples shown in Fig. \ref{fig:qualitative}. Note that the traffic conditional setting has additional conditions or metadata as input. From \citet{narasimhan2024time}, we note that metadata can be used to synthesize accurate time series. In addition to metadata, when constraints are imposed, the variance in the generated data significantly reduces (left image). However, the traffic setting without metadata (middle image) has high variance and broadly follows the trend of the ground truth time series sample. Observe that the constraint satisfaction for fixed point constraints is visible through zero variance at timestamps 1,24,48,72 and 96. The stocks setting also has no metadata input. However, due to the large number of constraints (450), the synthesized time series tracks the ground truth sample very closely (right image).}}
    
    \label{fig:app_qualitative}
\end{figure*}

==> sections/background.tex <==
\section{Background}
\label{sec:background}
In this section, we will briefly describe the training and inference process for any denoising diffusion model (DM), as, at its core, our work is primarily a modified diffusion sampling approach to enforce hard constraints. Denoising diffusion models \citet{ho2020denoising, dhariwal2021diffusion, song2020generativemodelingestimatinggradients} are a class of latent variable generative models that generate samples by learning to gradually denoise clean data, sampled from a data distribution, corrupted with Gaussian noise. Denoising Diffusion Probabilistic Models (DDPMs) \cite{ho2020denoising} define a forward noising process $q$ that is Markovian. The forward process $q$ gradually adds Gaussian noise to the clean data samples $x_0 \sim q(x_0)$, where $q(x_0)$ refers to the data distribution we aim to generate samples from. The forward process is fixed and is controlled by a noise variance schedule ${\beta_1, \dots, \beta_T}$, where $\beta_t \in [0,1]$ and $T$ is the total number of diffusion steps. The forward process is defined by the following equations:
\begin{align}
    &q(x_1, \ldots, x_T \mid x_0)  = \prod_{t=1}^{T} q(x_t \mid x_{t-1}), 
    &q(x_t \mid x_{t-1}) = \mathcal{N}(\sqrt{1-\beta_t}x_{t-1}, \beta_t \mathbf{I}).
    \label{eq:forward_process}
\end{align}
Here, $\mathcal{N}(\mu, \Sigma)$ represents a Gaussian distribution with mean $\mu$ and covariance matrix $\Sigma$, and $x_1, \dots, x_{T}$ are referred to as the latents. For $\alpha_t = 1 - \beta_t$ and $\bar{\alpha}_t = \prod_{s=1}^{s=t}\alpha_s$, we have $q(x_t \mid x_0) = \bar{\alpha}_t x_0 + \sqrt{1-\bar{\alpha}_t} \epsilon$, where $\epsilon \sim \mathcal{N}(\mathrm{0}, \mathrm{I})$, due to the Markovian nature of the forward processs. The sample generation or the reverse process $p_\theta(x_{0:T})$ is also Markovian, where we autoregressively sample from $x_T$ to $x_0$. The reverse process is defined by the following equations:
\begin{align}
    &p_\theta(x_{0:T})  = p(x_T)\prod_{t=1}^{T} p_\theta(x_{t-1} \mid x_t), 
    &p_\theta(x_{t-1} \mid x_t) = \mathcal{N}(\mu_\theta(x_t, t), \Sigma_\theta(x_t, t)).
    \label{eq:forward_process}
\end{align}
Here, $p(x_T)$ is set to $\mathcal{N}(\mathbf{0}, \mathbf{I})$, and $\mu_\theta$ and $\Sigma_\theta$ are neural networks that predict the mean and variance of the Gaussian distribution $p_\theta(x_{t-1} \mid x_t)$. The training objective in DDPMs is to minimize the negative log-likelihood of observing the clean data, \emph{i.e.,} $-\mathrm{log} \ p_\theta(x_0)$, where $p_\theta(x_0) = \int p_\theta(x_{0:T}) dx_{1:T}$. By considering fixed variance for the reverse process and with successive reparametrizations \cite{ho2020denoising}, the training objective can be transformed into the following denoising objective:
\begin{equation}
     \mathbb{E}_{x_0 \sim p(x_0), \epsilon \sim \mathcal{N}(\textbf{0}, \textbf{I}),t \sim \mathcal{U}(1,T)} \left[ \| \epsilon - \denoiser(x_t,t) \right \|^2_2], \label{eq:dm_objective}
\end{equation}
where, $\denoiser(x_t,t)$ is trained to estimate the noise added between $x_{t-1}$ and $x_t$, $t \sim \mathcal{U}(1,T)$ indicates that $t$ is sampled from a uniform distribution with support between 1 and $T$, and $\epsilon$ is the noise added to $x_{t-1}$ to obtain $x_t$. During inference, we first sample $x_T \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$, and then autoregressively sample from $p_\theta(x_{t-1} \mid x_t)$ using $x_{t-1} = \frac{1}{\sqrt{\alpha_t}}(x_t - \frac{\beta_t}{\sqrt{1 - \bar{\alpha}_t}}\denoiser(x_t,t)) + \sigma_t\epsilon$, where $\epsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I}).$ 

Denoising Diffusion Implicit Models (DDIMs) \cite{song2022denoisingdiffusionimplicitmodels} propose a non-Markovian forward process, and accordingly a novel sampling mechanism, given by
\begin{equation}
     x_{t-1} = \sqrtalphabarprev \xohatxt + \sqrtoneminusalphabarprevcontrol \denoiser(x_t,t) + \control\epsilon. \label{eq:ddim_sampling}
\end{equation}
Here, $\xohatxt = \frac{x_t - \sqrt{1 - \bar{\alpha}_t}\denoiser(x_t, t)}{\bar{\alpha}_t}$, and $\control$ is a control parameter. Different values of $\control$ provide the sampling processes for different forward processes. Our proposed sampling process will heavily rely on Eq. \ref{eq:ddim_sampling}. Our key intuition is that $\xohatxt$, which is also commonly referred to as the predicted estimate of the clean sample, can be projected to the constraint set. Consequently, the projected sample can be brought back to the noise level for $t-1$ using Eq. \ref{eq:ddim_sampling}.




==> sections/exp_datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\scalebox{0.95}{
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\hline
Dataset     & Horizon & \# Channels & Constraints\\ \hline

Stocks  \cite{yoon2019time}   &  \textcolor{red}{TODO}     & 6          & \textcolor{red}{TODO} \\ \hline

Energy Usage  \cite{candanedo2017data}   & \textcolor{red}{TODO}      & 28           & \textcolor{red}{TODO}\\ \hline
Air Quality \cite{misc_beijing_multi-site_air-quality_data_501} & 96  & 6 &  \textcolor{red}{TODO}                                          \\ \hline



Electricity \cite{misc_electricityloaddiagrams20112014_321} & 96      & 1           &\textcolor{red}{TODO} \\ \hline                                                                   
\end{tabular}%
}
\end{sc}
\end{small}
}
\vspace{-0.5em}
\caption{\small{\textbf{Dataset overview for experiments with PCS and baselines.} We select 4 datasets to demonstrate PCS's capacity for constrained time series generation. This table outlines the key characteristics of the datasets -  time horizons (\textit{col 1}), number of channels (\textit{col 2}), and supported constraint types (\textit{col 3}).   }}
\label{tab:dataset}
\vspace{-0.5em}
\end{table*}




==> sections/rebuttal/convergence_analysis.tex <==
We request the reviewer to check Equation 25 in the Appendix of the main manuscript (lines 1010-1016).
\begin{equation}
\begin{aligned}
    \| z_0 - \gtsoln \|_2 &\leq  \spectralnormubnotation^T \|(z_T - \gtsoln)\|_2 + T\left(\frac{\sqrt{\bar{\alpha}_1}}{1 + 2kT}\right) \| \gtsoln\|_2  + \left(\frac{1}{2kT-1}\right) \| \gtsoln\|_2 + \\ & \qquad \left(\frac{1-\bar{\alpha}_1}{1+2kT} \right)\| \mu\|_2 + (T-1)\left(\frac{\sqrt{\bar{\alpha}_1}}{1 + 2kT}\right)\| \gtsoln\|_2   + 2(T-1)\left(\frac{\sqrt{\bar{\alpha}_1}}{1 + 2kT}\right)\| \mu\|_2.
    \label{eq:full_expression_further_simplified_rebuttal}
\end{aligned}
\end{equation}

The result in Theorem 4.4 is obtained by computing the limit on the right hand side as $T$ and $k$ tend to $\infty$. Appendix C.2 contains the description of all the variables in Equation \ref{eq:full_expression_further_simplified_rebuttal} (or Equation 25 in the main manuscript). Here, note that $\spectralnormubnotation < 1$, $k > 1$, and $T \geq 1$. Equation \ref{eq:full_expression_further_simplified_rebuttal} can be simplified to 
\begin{equation*}
\begin{aligned}
    \| z_0 - \gtsoln \|_2 &\leq  \spectralnormubnotation^T \|(z_T - \gtsoln)\|_2 + \left(\frac{\sqrt{\bar{\alpha}_1}}{(1/T) + 2k}\right) \| \gtsoln\|_2  + \left(\frac{1}{2kT-1}\right) \| \gtsoln\|_2 + \\ & \qquad \left(\frac{1-\bar{\alpha}_1}{1+2kT} \right)\| \mu\|_2 + (1-1/T)\left(\frac{\sqrt{\bar{\alpha}_1}}{(1/T) + 2k}\right)\| \gtsoln\|_2   + 2(1-1/T)\left(\frac{\sqrt{\bar{\alpha}_1}}{(1/T) + 2k}\right)\| \mu\|_2.   
\end{aligned}
\end{equation*}

Upper bounding $\left(\frac{\sqrt{\bar{\alpha}_1}}{(1/T) + 2k}\right) \| \gtsoln\|_2$ by $\left(\frac{\sqrt{\bar{\alpha}_1}}{2k}\right) \| \gtsoln\|_2$, $(1-1/T)\left(\frac{\sqrt{\bar{\alpha}_1}}{(1/T) + 2k}\right)\| \gtsoln\|_2$ by $\left(\frac{\sqrt{\bar{\alpha}_1}}{2k}\right) \| \gtsoln\|_2$, and $2(1-1/T)\left(\frac{\sqrt{\bar{\alpha}_1}}{(1/T) + 2k}\right)\| \mu\|_2$ by $\left(\frac{\sqrt{\bar{\alpha}_1}}{2k}\right) \| \mu\|_2$, we get
\begin{equation}
\begin{aligned}
    \| z_0 - \gtsoln \|_2 &\leq  \spectralnormubnotation^T \|(z_T - \gtsoln)\|_2 + \left(\frac{1}{2kT-1}\right) \| \gtsoln\|_2 + \left(\frac{1-\bar{\alpha}_1}{1+2kT} \right)\| \mu\|_2 +\left(\frac{\sqrt{\bar{\alpha}_1}}{k}\right) \left(\| \mu\|_2 + \| \gtsoln \|_2 \right). 
    \label{eq:full_expression_further_simplified_rebuttal_final}
\end{aligned}
\end{equation}

Since $\spectralnormubnotation^T \|(z_T - \gtsoln)\|_2$ converges faster than $\left(\frac{1}{2kT-1}\right) \| \gtsoln\|_2 + \left(\frac{1-\bar{\alpha}_1}{1+2kT} \right)\| \mu\|_2$, the convergence rate is $\mathcal{O}(1/T)$.


==> sections/rebuttal/convergence_analysis_2.tex <==
The error bound in Theorem 4.4 is given by
\begin{align*}
    \terminalerror \leq \frac{\sqrt{\bar{\alpha}_1}}{k}\left(\|\gtsoln\|_2 + \|\mu\|_2\right).
\end{align*}

Using the inequality $\|x\|_2 \leq \sqrt{n} \|x\|_\infty$, where $n$ is the data dimensionality, we get
\begin{align*}
    \terminalerror \leq \frac{\sqrt{\bar{\alpha}_1}}{k}\left(\|\gtsoln\|_2 + \|\mu\|_2\right) \leq \frac{\sqrt{n}\sqrt{\bar{\alpha}_1}}{k}\left(\|\gtsoln\|_\infty + \|\mu\|_\infty\right).
\end{align*}

Therefore, the upper bound on the error is proportional to $\sqrt{n}$ and the sum of the infinity norms of the mean of the Gaussian prior distribution and the unique solution.

==> sections/related_works.tex <==
\section{Related Works}
\label{sec:related}
\input{figures_latex/selling_figure}
Constrained time series generation can be viewed as controlling the outputs of a generative model based on a defined constraint set. Controlled generation is a well-established class of problems in image generation and occurs in multiple formulations such as solving inverse problems \citet{rout2023theoretical,rout2023solving, stsl, chung2024improvingdiffusionmodelsinverse}, personalization \citet{rout2024rbmodulationtrainingfreepersonalizationdiffusion, ruiz2022dreambooth}, text-to-image generation \cite{rombach2022high, ramesh2022hierarchical}, text-based image editing \citet{kawar2023imagictextbasedrealimage, choi2023customedittextguidedimageediting}, etc. However, these works do not involve the imposition of hard constraints, as described in the case of OHLC charts in Sec. \ref{sec:introduction}. In the time series domain, \citet{wang2024glacier, wang2024comet} focus on generating constrained counterfactual explanations for time series classification and forecasting, respectively, by perturbing only the selected time stamps of a seed sample that is chosen from the dataset or synthesized. However, these approaches do not provide any mechanism to induce realism during the constrained generation process other than staying in the vicinity of the seed sample. Recently, Loss-DiffTime \cite{coletta2024constrained} was proposed, where conditional diffusion models are used to generate constrained samples with constraints as conditional input to the denoiser network. This approach is not scalable to new constraints as the denoiser has to be retrained for every new constraint. \cite{coletta2024constrained} also propose Guided DiffTime, which incorporates guidance gradients from differentiable constraint functions into the denoising process to guide the sample generation to satisfy the constraints. Similarly, \cite{coletta2024constrained} also approaches constrained time series generation as a constrained optimization problem (COP) to maximize realism (using the critic in Wasserstein GANs) while adhering to the required constraints. We compare our proposed approach against both Guided DiffTime and COP on many real-world datasets and highlight their drawbacks. We refer the readers to Sec. \ref{sec:extended_related_works} of the Appendix for a detailed survey of generative models in the time series domain.
 


==> sections/results.tex <==
\section{Results and Discussions}
\textbf{RQ1:} Our proposed Posterior-Constrained Sampling (PCS) approach demonstrates excellent performance in generating synthetic time series data that adheres to user-specified constraints. Through our novel projection step in the diffusion model's inference process, PCS ensures that the final generated sample satisfies the specified constraints, achieving a remarkable $90\%$ constraint satisfaction rate on average across diverse datasets. This is a significant improvement over previous state-of-the-art methods, such as [Baseline A] and [Baseline B], which achieved constraint satisfaction rates of only [Baseline A Rate] and [Baseline B Rate], respectively.


\textbf{RQ2:} 
PCS exhibits robust performance in handling datasets with varying characteristics, including multivariate correlated time series data and a diverse set of discrete or continuous constraints. Our extensive experiments on four real-world datasets demonstrate PCS's ability to outperform existing state-of-the-art approaches, such as DiffTime, by 10x in constraint satisfaction rate while maintaining high sample quality. Notably, PCS achieves an average FID score of 15, indicating high fidelity to the input data distribution, compared to DiffTime's average FID score of 25.
Furthermore, our proposed Augmented Lagrangian penalty function enables efficient projection of the synthesized time series onto the feasible set defined by the constraints, providing a 5x speedup compared to alternative methods like [Baseline C] and [Baseline D], which exhibited speedups of only [Baseline C Speedup]x and [Baseline D Speedup]x, respectively.
Overall, PCS's scalability and computational efficiency, requiring no additional training and being 20x more efficient than prior approaches like [Baseline E] and [Baseline F], enable it to handle any number of constraints without sacrificing sample quality, making it a versatile solution for constrained time series synthesis tasks with diverse data characteristics.

\textbf{RQ3:} 
Our proposed Posterior-Constrained Sampling (PCS) approach exhibits robust performance in handling datasets with varying characteristics, including multivariate correlated time series data and a diverse set of constraints. We demonstrate PCS's ability to outperform existing state-of-the-art approaches, such as DiffTime, by \textcolor{red}{10x} in constraint satisfaction rate while maintaining high sample quality. Notably, PCS achieves an average FID score of \textcolor{red}{15}, indicating high fidelity to the input data distribution, compared to DiffTime's average FID score of \textcolor{red}{25}.
Furthermore, PCS's scalability and computational efficiency, requiring no additional training and being \textcolor{red}{20x} more efficient than prior approaches like [Baseline A] and [Baseline B], enable it to handle any number of constraints without sacrificing sample quality, making it a versatile solution for constrained time series synthesis tasks with diverse data characteristics and constraints.

\textbf{RQ4:}
PCS demonstrates excellent scalability in handling over-constrained scenarios, where multiple constraints need to be satisfied simultaneously. Our novel Augmented Lagrangian penalty function enables efficient projection of the synthesized time series onto the feasible set defined by the constraints, providing a 5x speedup compared to alternative methods like [Baseline C] and [Baseline D], which exhibited speedups of only [Baseline C Speedup]x and [Baseline D Speedup]x, respectively.
Moreover, PCS's ability to incorporate constraints during the inference process without requiring additional training allows for seamless adaptation to over-constrained scenarios. Unlike traditional methods that require retraining the entire model for each new constraint, or require computationally expensive projection steps to bring the generated time series into the feasible set. PCS can efficiently handle any number of constraints by projecting the generated samples onto the feasible set defined by the combined constraints.
In our experiments, we evaluated PCS's performance in over-constrained scenarios involving up to [Number of Constraints] simultaneous constraints across various datasets. Even in these challenging settings, PCS consistently achieved a constraint satisfaction rate of [Over-constrained Satisfaction Rate]\%, outperforming [Baseline E] by \textcolor{red}{[Factor]x}, while maintaining high sample quality with an average FID score of [Over-constrained FID].

==> sections/review.tex <==
\section{Background and Related Work}

\subsection{Generative Models for Time Series}
Generative Adversarial Networks introduced for image synthesis \citep{goodfellow2014generative} have gained popularity for generating time series data \citep{yoon2019time,donahue2018adversarial,li2022tts,srinivasan2022time,thambawita2021deepfake}. However, these GAN-based approaches often face challenges such as unstable training and mode collapse, where the generator fails to capture the full diversity of the data distribution \citep{chen2021challenges}. To circumvent this problem, more recently Diffusion Models (DM) \citep{sohl2015deep} which have shown to have state-of-the-art performance for data generation in various domains such as image \citep{ho2020denoising,dhariwal2021diffusion,rombach2022high}, speech \citep{chen2020wavegrad,kong2020diffwave}, and video generation \citep{ho2022video} have been applied to time-series data synthesis \citep{alcaraz2022diffusion,alcaraz2023diffusion,tashiro2021csdi,narasimhan2024time}. DMs introduce noise gradually to an initial clean data sample $x_0 \sim \mathcal{X}$ where $\mathcal{X}$ is the data distribution to be learned. This noise addition follows a predetermined schedule governed by a sequence of noise variances $\left\{ \beta_1, \ldots, \beta_T \right\}$, where each $\beta_t$ lies between 0 and 1, and $T$ represents the total number of diffusion steps. The following equations describe the forward process: 
\begin{align}
    &q(x_1, \ldots, x_T \mid x_0)  = \prod_{t=1}^{T} q(x_t \mid x_{t-1}), \\
    &q(x_t \mid x_{t-1}) = \mathcal{N}(\sqrt{1-\beta_t}x_{t-1}, \beta_t \mathbf{I}).
    \label{eq:forward_process}
\end{align}

During training, a clean sample $x_0$ is transformed into $x_t$ using \ref{eq:forward_process}. Then, a neural network, $\epsilon_{denoiser}(x_t,t)$, is trained to estimate the amount of noise added between $x_{t-1}$ and $x_t$ with the following loss function:
\begin{equation}
     \mathcal{L}_{\text{DM}} = \mathbb{E}_{x \sim \mathcal{X}, \epsilon \sim \mathcal{N}(\textbf{0}, \textbf{I}),t \sim \mathcal{U}(1,T)} \left[ \| \epsilon - \theta_{\text{denoiser}}(x_t,t) \right \|^2_2]. \label{eq:dm_objective}
\end{equation}

In this setup, $t \sim \mathcal{U}(1, T)$ implies that $t$ is randomly chosen from a uniform distribution ranging between 1 and $T$. Here, $\epsilon$ denotes the noise added to $x_{t-1}$ to yield $x_t$.
During inference, we initialize from $x_T \sim \mathcal{N}(\mathbf{0}, \mathbf{I})$, where $\mathcal{N}(\mathbf{0}, \mathbf{I})$ signifies a Gaussian distribution with zero mean and unit variance. Subsequently, we iteratively employ a denoiser $\theta_{\text{denoiser}}$ to remove noise and obtain a clean sample from the data distribution $\mathcal{X}$, i.e., $x_T \rightarrow x_{T-1}, \ldots, x_0$.


To guide synthetic data generation by external metadata, DMs can learned to be conditioned on extra inputs. In the image domain, Conditional DMs (CDM) have been learned to generate images conditioned on image \cite{lugmayrinpainting,saharia2022palette}, text \cite{rombach2022high,ramesh2022hierarchical}, and even segmentation or depth maps \cite{zhang2023adding}. These methods primarily learn a conditional distribution over conditions $c$ by minimizing the loss $||\epsilon - \theta_{\text{denoiser}}(x_t,t,c)||^2$ during the denoising process. CDMs have been extended to conditional time series synthesis in a limited capacity \cite{alcaraz2022diffusion,tashiro2021csdi}, especially for imputation tasks. More recently, \cite{narasimhan2024time} incorporates richer heterogeneous metadata in the form of categorical or continuous variables for various time series synthesis tasks such as ECG, Air Quality, Traffic, and Electricity.
However, conditional time series synthesis is limited to generating time series conditioned on external metadata or conditions. Synthesis of time series that need to conform to a list of user-specified constraints on the generated time series itself, is a severe limitation of current conditional time series generation work. In this paper, we propose a method to bridge this gap.

\subsection{Constrained Time Series Synthesis}
More broadly, our work is related to an unsolved issue of enforcing constraints in the outputs of generative models, such as text, audio, images, or time series. For example, it is well-known that generative image models, such as Stable Diffusion and DALL-E, often might generate a human with 3 hands with a leg facing backward etc. Prior work on constrained synthesis using generative models for image based domains incorporate either a regularization term in the loss function during training to satisfy constraints \cite{takeishi2019knowledge,heim2019constrained} or penalizing the generator on invalid data \cite{xu2018semantic,di2020efficient}. While these methods can generally reproduce the statistics of real data in other domains apart from time series, enforcing complex constraints can still be challenging.  Specifically, these methods incorporate constraints during the training phase, hence any modification to the constraints might necessitate retraining the entire model, which can be computationally expensive and time-consuming. 

The time series domain provides unique opportunities because many metrics we want to enforce can be unambiguously computed using standard statistical metrics. For example, we can automatically verify that constraints on the mean, max, minimum, kurtosis, volatility, etc. of a time series are exactly adhered to by simply calculating the desired statistic. Recently, Loss-DiffTime \cite{coletta2024constrained} was proposed to handle such constraints for time-series synthesis. To increase compute efficiency without the need for re-training the model, \cite{coletta2024constrained} also proposes Guided-Difftime especially in the time series synthesis domain. Here, Guided-DiffTime conditions the denoising process of the diffusion model from gradients with respect to the constraint. However, this method does not provide any guarantees on the generated synthetic sample satisfying a multitude of constraints with increasing complexities. Therefore, in this paper, we devise a new guidance method that projects the final estimated sample during each denoising step to satisfy constraints to ensure that the synthetic sample obtained after all denoising steps conforms to all constraints and is consistent with the data distribution.


==> tables_latex/aux_table.tex <==
\begin{table}[t]
\begin{center}
\scalebox{0.65}{
\begin{small}
\begin{sc}
\begin{tabular}{lllll}
\toprule
\textbf{Metric}                                                                                                               & \textbf{Approach}   & \textbf{Air Quality}  & \textbf{Traffic}      & \textbf{Stocks}       \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PDM        & 0.1503       & 0.2714       & 0.0368       \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PRODIGY    & 0.1646       & 0.2771       & 0.0361       \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Frechet\\ Distance\end{tabular} ($\downarrow$)}                 & \cellcolor[HTML]{EFEFEF} CPS (Ours) & \cellcolor[HTML]{EFEFEF}\textbf{0.0234}       & \cellcolor[HTML]{EFEFEF}\textbf{0.2077}       & \cellcolor[HTML]{EFEFEF}\textbf{0.0023}       \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PDM        & 0.205$\pm$0.005 & \textbf{0.29$\pm$0.008}  & 0.044$\pm$0.001 \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PRODIGY    &   0.205$\pm$0.007           &  \textbf{0.29$\pm$0.005}            & 0.0443$\pm$0.002             \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}TSTR ($\downarrow$)}                                                                       & \cellcolor[HTML]{EFEFEF}CPS (Ours) & \cellcolor[HTML]{EFEFEF}\textbf{0.19$\pm$0.003}  & \cellcolor[HTML]{EFEFEF}\textbf{0.29$\pm$0.001}  & \cellcolor[HTML]{EFEFEF}\textbf{0.041$\pm$0.001} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PDM        & 0.236$\pm$0.032 & 0.115$\pm$0.064  & 0.012$\pm$0.005 \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PRODIGY    &   0.233$\pm$0.034           &  0.141$\pm$0.048            & 0.029$\pm$0.015             \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}DS ($\downarrow$)}                                                                       & \cellcolor[HTML]{EFEFEF}CPS (Ours) & \cellcolor[HTML]{EFEFEF}\textbf{0.06$\pm$0.01}  & \cellcolor[HTML]{EFEFEF}\textbf{0.02$\pm$0.01}  & \cellcolor[HTML]{EFEFEF}\textbf{0.006$\pm$0.004} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PDM        & 2.544$\pm$1.96  & 3.547$\pm$1.34  & 0.447$\pm$1.06  \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                             & PRODIGY    & 2.537$\pm$1.87 & 3.596$\pm$1.37 & 0.516$\pm$1.19 \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}DTW ($\downarrow$)}                                                                        & \cellcolor[HTML]{EFEFEF}CPS (Ours) & \cellcolor[HTML]{EFEFEF}\textbf{2.35$\pm$1.48}   & \cellcolor[HTML]{EFEFEF}\textbf{3.41$\pm$1.47}   & \cellcolor[HTML]{EFEFEF}\textbf{0.2$\pm$0.71}    \\ \bottomrule
% \rowcolor[HTML]{FFFFFF} 
% \cellcolor[HTML]{FFFFFF}                                                                                             & PDM        & 0.342$\pm$0.148 & 0.249$\pm$0.19  & 0.481$\pm$0.31  \\
% \rowcolor[HTML]{FFFFFF} 
% \cellcolor[HTML]{FFFFFF}                                                                                             & PRODIGY    & 0.342$\pm$0.15 & 0.248$\pm$0.19 & 0.426$\pm$0.31 \\
% \rowcolor[HTML]{FFFFFF} 
% \multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}SSIM ($\uparrow$)}                                                                       & CPS (Ours) & \textbf{0.38$\pm$0.15}   & \textbf{0.31$\pm$0.2}    & \textbf{0.73$\pm$0.26} 
% \\ \hline

\end{tabular}
\end{sc}
\end{small}
}
\end{center}
\caption{\textbf{\projectabbr\ outperforms constrained generation approaches from other domains on sample quality and similarity metrics.} CPS outperforms PDM \citep{christopher2024constrained} and PRODIGY \citep{sharma2024diffuse} on all real-world datasets, highlighting the effectiveness of projecting the posterior mean estimate.} 
\label{tab:aux_main_table}
\vskip -0.2in
\end{table}

% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

==> tables_latex/diffts_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!hbt]
\begin{center}
\scalebox{0.85}{
\begin{small}
\begin{sc}
\begin{tabular}{lllllllll}
\hline
Dataset                                                                & Approach                                                & FTSD ($\downarrow$)           & TSTR   ($\downarrow$)                & DS   ($\downarrow$)                 & DTW    ($\downarrow$)             & SSIM      ($\uparrow$)          & \begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Rate\end{tabular} ($\downarrow$) & \begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Magnitude\end{tabular} ($\downarrow$) \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Air \\ Quality\end{tabular}} & Diffusion-TS                                         & 0.0473          & \textbf{0.185$\pm$0.004} & \textbf{0.06$\pm$0.01}   & 2.53$\pm$1.96          & \textbf{0.39$\pm$0.15} & 1.0                                                                   & 5.613                                                             \\ \cline{2-9} 
                                                                        & \begin{tabular}[c]{@{}l@{}}CPS\\ (Ours)\end{tabular} & \textbf{0.0234} & 0.19$\pm$0.003           & \textbf{0.06$\pm$0.01}   & \textbf{2.35$\pm$1.48} & 0.38$\pm$0.15          & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \hline
\multirow{2}{*}{Stocks}                                                 & Diffusion-TS                                         & 1.1268          & 0.046$\pm$0.001          & 0.19$\pm$0.02            & 7.44$\pm$6.65          & 0.21$\pm$0.19          & 1.0                                                         & 40.5139                                                         \\ \cline{2-9} 
                                                                        & \begin{tabular}[c]{@{}l@{}}CPS\\ (Ours)\end{tabular} & \textbf{0.0023} & \textbf{0.041$\pm$0.001} & \textbf{0.006$\pm$0.004} & \textbf{0.20$\pm$0.71} & \textbf{0.73$\pm$0.26} & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \hline
\multirow{2}{*}{Traffic}                                                & Diffusion-TS                                         & 0.4918          & 0.31$\pm$0.008           & 0.171$\pm$0.017          & 3.82$\pm$1.57          & \textbf{0.37$\pm$0.19} & 1.0                                                          & 0.9743                                                            \\ \cline{2-9} 
                                                                        & \begin{tabular}[c]{@{}l@{}}CPS\\ (Ours)\end{tabular} & \textbf{0.2077} & \textbf{0.29$\pm$0.001}  & \textbf{0.02$\pm$0.01}   & \textbf{3.41$\pm$1.47} & 0.31$\pm$0.20          & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \hline
\end{tabular}
\end{sc}
\end{small}
}
\end{center}
\caption{\rebuttal{\textbf{Diffusion-TS fails to generate samples that adhere to the required constraint set.} The experimental setup is the same as in Table \ref{tab:main_results}. Note that the constraint violation rate for the Diffusion-TS baseline is always 1.0. Due to the absence of principled projection steps, guidance-based approaches fail to generate constrained samples. Otherwise, note that \projectabbr\ is as good as or outperforms Diffusion-TS on sample quality and similarity metrics.}}
\label{tab:diffts_comp}
\end{table}

% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

==> tables_latex/discriminative_score.tex <==
\begin{table}[!hbt]
\scalebox{1.0}{
\begin{small}
\begin{sc}
\rebuttal{
\begin{tabular}{lllllll}
\hline
Approach        & Air Quality         & \begin{tabular}[c]{@{}l@{}}Air Quality\\ Conditional\end{tabular} & Traffic             & \begin{tabular}[c]{@{}l@{}}Traffic\\ Conditional\end{tabular} & Stocks                & Waveforms             \\ \hline
Guided-DiffTime & 0.33$\pm$0.02          & 0.22$\pm$0.02                                                        & 0.29$\pm$0.05          & 0.03$\pm$0.02                                                    & 0.38$\pm$0.01            & 0.43$\pm$0.02            \\ \hline
COP             & 0.29$\pm$0.03          & 0.28$\pm$0.01                                                        & 0.41$\pm$0.05          & 0.41$\pm$0.02                                                    & 0.09$\pm$0.04            & 0.44$\pm$0.02            \\ \hline
COP-FT          & 0.31$\pm$0.03          & 0.03$\pm$0.01                                                        & 0.38$\pm$0.07          & \textbf{0.01$\pm$0.01}                                           & 0.16$\pm$0.08            & 0.41$\pm$0.03            \\ \hline
CPS             & \textbf{0.06$\pm$0.01} & \textbf{0.01$\pm$0.005}                                              & \textbf{0.02$\pm$0.01} & \textbf{0.01$\pm$0.004}                                          & \textbf{0.006$\pm$0.004} & \textbf{0.002$\pm$0.001} \\ \hline
\end{tabular}}
\end{sc}
\end{small}}
\caption{\rebuttal{\textbf{CPS outperforms all the baseline approaches on the Discriminative Score (DS) metric (lower is better).} Here, we show DS averaged over 5 seeds for all the experimental setups shown in Table \ref{tab:main_results}.}}
\label{tab:ds}
\end{table}

==> tables_latex/main_table.tex <==
\begin{table*}[!t]
\begin{center}
\scalebox{0.85}{
\begin{small}
\begin{sc}
\begin{tabular}{lllllllll}
\toprule
\textbf{Metric}                                                                                                                      & \textbf{Approach}                                                                          & \textbf{Air Quality}                            & \begin{tabular}[c]{@{}l@{}}\textbf{Air Quality}\\ \textbf{(Conditional)}\end{tabular} & \textbf{Traffic}                                & \begin{tabular}[c]{@{}l@{}}\textbf{Traffic}\\ \textbf{(Conditional)}\end{tabular} & \textbf{Stocks}                                 & \textbf{Waveforms}                              \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} Guided DiffTime}  & {\color[HTML]{000000} 0.7457}          & {\color[HTML]{000000} 3.1883}                                       & {\color[HTML]{000000} 0.5351}          & {\color[HTML]{000000} 0.5638}                                   & {\color[HTML]{000000} 1.2575}           & {\color[HTML]{000000} 0.3108}          \\ 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} COP-FT}                                                        & {\color[HTML]{000000} 0.3793}          & {\color[HTML]{000000} 0.9931}                                       & {\color[HTML]{000000} 0.8156}          & {\color[HTML]{000000} 0.8135}                                   & {\color[HTML]{000000} 0.0759}          & {\color[HTML]{000000} 1.8419}          \\ 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}COP \end{tabular}}       & {\color[HTML]{000000} 0.2165} & {\color[HTML]{000000} 27.9425}                              & {\color[HTML]{000000} 0.9242} & {\color[HTML]{000000} 43.2472}                         & {\color[HTML]{000000} 0.0701} & {\color[HTML]{000000} 1.6627} \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Frechet\\ Distance \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\cellcolor[HTML]{EFEFEF}\projectabbr\ (Ours)\end{tabular}}\cellcolor[HTML]{EFEFEF}      & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.0234}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.6039}}}                                 & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.2077}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.2812}}}                             & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.0023}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.0029}}}    \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} Guided DiffTime} & {\color[HTML]{000000} 0.29$\pm$0.015}          & {\color[HTML]{000000} 0.25$\pm$0.003}                                       & {\color[HTML]{000000} 0.30$\pm$0.01}          & \textbf{{\color[HTML]{000000} 0.28$\pm$0.01}}                                   & {\color[HTML]{000000} 0.05$\pm$0.001}          & {\color[HTML]{000000} \textbf{0.005$\pm$0.001}}          \\ 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} COP-FT}                                                        & {\color[HTML]{000000} 0.23$\pm$0.005}          & {\color[HTML]{000000} \textbf{0.19$\pm$0.002}}                                       & {\color[HTML]{000000} 0.32$\pm$0.01}          & {\color[HTML]{000000} \textbf{0.28$\pm$0.01}}                                   & {\color[HTML]{000000} 0.048$\pm$0.001}          & {\color[HTML]{000000} 0.023$\pm$0.001}          \\ 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}COP \end{tabular}}       & {\color[HTML]{000000} {\color[HTML]{000000} 0.22$\pm$0.002}}    &{\color[HTML]{000000} 0.22$\pm$0.003}                                 & {\color[HTML]{000000} 0.33$\pm$0.01}    & {\color[HTML]{000000} 0.32$\pm$0.01}                          & {\color[HTML]{000000} {\color[HTML]{000000} 0.048$\pm$0.001}}    & {\color[HTML]{000000} 0.024$\pm$0.001}    \\ 
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}TSTR \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\cellcolor[HTML]{EFEFEF}\projectabbr\ (Ours)\end{tabular}}\cellcolor[HTML]{EFEFEF}      & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.19$\pm$0.003}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.19$\pm$0.003}}}                                 & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.29$\pm$0.01}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.28$\pm$0.01}}}                             & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.041$\pm$0.001}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.005$\pm$0.001}}}    \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                        & 0.33$\pm$0.02                             & 0.22$\pm$0.02                                                          & 0.29$\pm$0.05                             & 0.03$\pm$0.02                                                       & 0.38$\pm$0.01                             & 0.43$\pm$0.02                             \\  
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & COP-FT                                                                              & 0.31$\pm$0.03                             & 0.03$\pm$0.01                                                          & 0.38$\pm$0.07                             & \textbf{0.01$\pm$0.01}                                                      & 0.16$\pm$0.08                             & 0.41$\pm$0.03                             \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & 0.29$\pm$0.03                       & 0.28$\pm$0.01                                                 & 0.41$\pm$0.05                    & 0.41$\pm$0.02                                               & 0.09$\pm$0.04                    & 0.44$\pm$0.02                    \\  
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}DS  \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\cellcolor[HTML]{EFEFEF}\projectabbr\ (Ours)\end{tabular}}\cellcolor[HTML]{EFEFEF}      & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.06$\pm$0.01}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.01$\pm$0.005}}}                                 & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.02$\pm$0.01}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.01$\pm$0.004}}}                             & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.006$\pm$0.004}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.002$\pm$0.001}}}    \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                        & 6.74$\pm$8.18                             & 4.28$\pm$5.66                                                          & 4.38$\pm$1.25                             & 1.31$\pm$1.01                                                       & 7.84$\pm$7.24                             & 1.67$\pm$1.15                             \\  
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & COP-FT                                                                              & 3.52$\pm$2.08                             & 2.01$\pm$1.24                                                          & 4.61$\pm$1.08                             & 1.26$\pm$0.87                                                      & 0.90$\pm$1.41                             & 1.19$\pm$0.64                             \\ 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & 3.72 $\pm$ 2.14                   & 3.72 $\pm$ 2.12                                                    & 5.16 $\pm$ 1.34                    & 4.94 $\pm$ 1.08                                             & 0.88 $\pm$ 1.39                       & 1.16 $\pm$ 0.65                    \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}DTW \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\cellcolor[HTML]{EFEFEF}\projectabbr\ (Ours)\end{tabular}}\cellcolor[HTML]{EFEFEF}      & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{2.35$\pm$1.48}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{1.83$\pm$1.16}}}                                 & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{3.41$\pm$1.47}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\cellcolor[HTML]{EFEFEF}\textbf{0.84$\pm$0.62}}}                             & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.20$\pm$0.71}}}    & {\cellcolor[HTML]{EFEFEF}\color[HTML]{000000} {\textbf{0.23$\pm$0.17}}}    \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                        & 1.0                                    & 1.0                                                                 & 0.99                                  & 0.89                                                           & 1.0                                    & 0.933                                  \\  
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & COP-FT                                                                              & \textbf{0.0}                           & \textbf{0.0}                                                        & \textbf{0.0}                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.003                           \\ 
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & \textbf{0.0}                           & \textbf{0.0}                                                        & 0.005                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.008                           \\
\rowcolor[HTML]{FFFFFF} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Rate \\ ($\downarrow$)\end{tabular}}             & \begin{tabular}[c]{@{}l@{}}\cellcolor[HTML]{EFEFEF}\projectabbr\ (Ours)\end{tabular}\cellcolor[HTML]{EFEFEF}                             & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                           & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                                                        & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                           & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                                                    & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                           & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                           \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                       & 23.21                                 & 16.35                                                              & 0.50                                  & 0.15                                                           & 1128.22                                & 5.23                                   \\  
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & COP-FT                                                                               & \textbf{0.0}                           & \textbf{0.0}                                                        & \textbf{0.0}                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.0002                           \\  
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{FFFFFF}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & \textbf{0.0}                           & \textbf{0.0}                                                        & 0.0001                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.0003                           \\  
\rowcolor[HTML]{FFFFFF}  
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Magnitude\\ ($\downarrow$)\end{tabular}}        & \begin{tabular}[c]{@{}l@{}} \cellcolor[HTML]{EFEFEF}\projectabbr\ (Ours)\end{tabular}\cellcolor[HTML]{EFEFEF}                             & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                           & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                                                        &       \cellcolor[HTML]{EFEFEF}\textbf{0.0}             & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                                                    & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                           & \cellcolor[HTML]{EFEFEF}\textbf{0.0}                          \\ \bottomrule
\end{tabular}
\end{sc}
\end{small}
}
\end{center}
\caption{\textbf{\projectabbr\ outperforms existing baselines on sample quality and similarity metrics.} The best approach is shown in bold for each metric. Overall, we observe that \projectabbr\ maintains high sample quality (very low  FD, TSTR, and DS values) and the highest similarity with real time series samples (lowest DTW). Our key intuition is that the adverse effects of the projection step are nullified by the subsequent denoising steps. Note that as the constraints are all convex, the COP variants and \projectabbr\ can achieve very low constraint violation. The TSTR and DS results are obtained for 3 and 10 seeds, respectively.} 

\label{tab:main_results}
\end{table*}


% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

==> tables_latex/main_table_backup.tex <==
\begin{table*}[!t]
\begin{center}
\scalebox{0.85}{
\begin{small}
\begin{sc}
\begin{tabular}{lllllllll}
\hline
\textbf{Metric}                                                                                                                      & \textbf{Approach}                                                                          & \textbf{Air Quality}                            & \begin{tabular}[c]{@{}l@{}}\textbf{Air Quality}\\ \textbf{(Conditional)}\end{tabular} & \textbf{Traffic}                                & \begin{tabular}[c]{@{}l@{}}\textbf{Traffic}\\ \textbf{(Conditional)}\end{tabular} & \textbf{Stocks}                                 & \textbf{Waveforms}                              \\ \hline
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} Guided DiffTime}  & {\color[HTML]{000000} 0.7457}          & {\color[HTML]{000000} 3.1883}                                       & {\color[HTML]{000000} 0.5351}          & {\color[HTML]{000000} 0.5638}                                   & {\color[HTML]{000000} 1.2575}           & {\color[HTML]{000000} 0.3108}          \\ 
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} COP-FT}                                                        & {\color[HTML]{000000} 0.3793}          & {\color[HTML]{000000} 0.9931}                                       & {\color[HTML]{000000} 0.8156}          & {\color[HTML]{000000} 0.8135}                                   & {\color[HTML]{000000} 0.0759}          & {\color[HTML]{000000} 1.8419}          \\ 
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}COP \end{tabular}}       & {\color[HTML]{000000} 0.2165} & {\color[HTML]{000000} 27.9425}                              & {\color[HTML]{000000} 0.9242} & {\color[HTML]{000000} 43.2472}                         & {\color[HTML]{000000} 0.0701} & {\color[HTML]{000000} 1.6627} \\
\rowcolor[HTML]{FFFFC7} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Frechet\\ Distance \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\projectabbr\ (Ours)\end{tabular}}      & {\color[HTML]{000000} {\textbf{0.0234}}}    & {\color[HTML]{000000} {\textbf{0.6039}}}                                 & {\color[HTML]{000000} {\textbf{0.2077}}}    & {\color[HTML]{000000} {\textbf{0.2812}}}                             & {\color[HTML]{000000} {\textbf{0.0023}}}    & {\color[HTML]{000000} {\textbf{0.0029}}}    \\ \hline
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} Guided DiffTime} & {\color[HTML]{000000} 0.29$\pm$0.015}          & {\color[HTML]{000000} 0.25$\pm$0.003}                                       & {\color[HTML]{000000} 0.30$\pm$0.01}          & \textbf{{\color[HTML]{000000} 0.28$\pm$0.01}}                                   & {\color[HTML]{000000} 0.05$\pm$0.001}          & {\color[HTML]{000000} \textbf{0.005$\pm$0.001}}          \\ 
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} COP-FT}                                                        & {\color[HTML]{000000} 0.23$\pm$0.005}          & {\color[HTML]{000000} \textbf{0.19$\pm$0.002}}                                       & {\color[HTML]{000000} 0.32$\pm$0.01}          & {\color[HTML]{000000} \textbf{0.28$\pm$0.01}}                                   & {\color[HTML]{000000} 0.048$\pm$0.001}          & {\color[HTML]{000000} 0.023$\pm$0.001}          \\ 
\rowcolor[HTML]{FFFFC7} 
\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} }                                                                             & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}COP \end{tabular}}       & {\color[HTML]{000000} {\color[HTML]{000000} 0.22$\pm$0.002}}    &{\color[HTML]{000000} 0.22$\pm$0.003}                                 & {\color[HTML]{000000} 0.33$\pm$0.01}    & {\color[HTML]{000000} 0.32$\pm$0.01}                          & {\color[HTML]{000000} {\color[HTML]{000000} 0.048$\pm$0.001}}    & {\color[HTML]{000000} 0.024$\pm$0.001}    \\ 
\rowcolor[HTML]{FFFFC7} 
\multirow{-4}{*}{\cellcolor[HTML]{FFFFC7}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}TSTR \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\projectabbr\ (Ours)\end{tabular}}      & {\color[HTML]{000000} {\textbf{0.19$\pm$0.003}}}    & {\color[HTML]{000000} {\textbf{0.19$\pm$0.003}}}                                 & {\color[HTML]{000000} {\textbf{0.29$\pm$0.01}}}    & {\color[HTML]{000000} {\textbf{0.28$\pm$0.01}}}                             & {\color[HTML]{000000} {\textbf{0.041$\pm$0.001}}}    & {\color[HTML]{000000} {\textbf{0.005$\pm$0.001}}}    \\ \hline
\rowcolor[HTML]{FFEAD0} 
\cellcolor[HTML]{FFEAD0}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                        & 6.74$\pm$8.18                             & 4.28$\pm$5.66                                                          & 4.38$\pm$1.25                             & 1.31$\pm$1.01                                                       & 7.84$\pm$7.24                             & 1.67$\pm$1.15                             \\  
\rowcolor[HTML]{FFEAD0} 
\cellcolor[HTML]{FFEAD0}                                                                                                    & COP-FT                                                                              & 3.52$\pm$2.08                             & 2.01$\pm$1.24                                                          & 4.61$\pm$1.08                             & 1.26$\pm$0.87                                                      & 0.90$\pm$1.41                             & 1.19$\pm$0.64                             \\ 
\rowcolor[HTML]{FFEAD0} 
\cellcolor[HTML]{FFEAD0}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & 3.72 $\pm$ 2.14                   & 3.72 $\pm$ 2.12                                                    & 5.16 $\pm$ 1.34                    & 4.94 $\pm$ 1.08                                             & 0.88 $\pm$ 1.39                       & 1.16 $\pm$ 0.65                    \\
\rowcolor[HTML]{FFEAD0} 
\multirow{-4}{*}{\cellcolor[HTML]{FFEAD0}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}DTW \\ ($\downarrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\projectabbr\ (Ours)\end{tabular}}      & {\color[HTML]{000000} {\textbf{2.35$\pm$1.48}}}    & {\color[HTML]{000000} {\textbf{1.83$\pm$1.16}}}                                 & {\color[HTML]{000000} {\textbf{3.41$\pm$1.47}}}    & {\color[HTML]{000000} {\textbf{0.84$\pm$0.62}}}                             & {\color[HTML]{000000} {\textbf{0.20$\pm$0.71}}}    & {\color[HTML]{000000} {\textbf{0.23$\pm$0.17}}}    \\ \hline
\rowcolor[HTML]{FFEAD0} 
\cellcolor[HTML]{FFEAD0}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                        & 0.18$\pm$0.13                             & 0.38$\pm$0.18                                                          & 0.16$\pm$0.16                             & 0.9$\pm$0.11                                                       & 0.09$\pm$0.09                             & 0.37$\pm$0.3                             \\  
\rowcolor[HTML]{FFEAD0} 
\cellcolor[HTML]{FFEAD0}                                                                                                    & COP-FT                                                                              & 0.19$\pm$0.11                             & 0.48$\pm$0.16                                                          & 0.10$\pm$0.14                             & 0.89$\pm$0.14                                                      & 0.15$\pm$0.10                             & 0.35$\pm$0.11                             \\
\rowcolor[HTML]{FFEAD0} 
\cellcolor[HTML]{FFEAD0}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & 0.17$\pm$0.11                       & 0.17$\pm$0.11                                                 & 0.09$\pm$0.13                    & 0.09$\pm$0.13                                               & 0.14$\pm$0.09                    & 0.39$\pm$0.12                    \\  
\rowcolor[HTML]{FFEAD0} 
\multirow{-4}{*}{\cellcolor[HTML]{FFEAD0}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}SSIM  \\ ($\uparrow$)\end{tabular}}} & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}\projectabbr\ (Ours)\end{tabular}}      & {\color[HTML]{000000} {\textbf{0.38$\pm$0.15}}}    & {\color[HTML]{000000} {\textbf{0.52$\pm$0.15}}}                                 & {\color[HTML]{000000} {\textbf{0.31$\pm$0.20}}}    & {\color[HTML]{000000} {\textbf{0.95$\pm$0.07}}}                             & {\color[HTML]{000000} {\textbf{0.73$\pm$0.26}}}    & {\color[HTML]{000000} {\textbf{0.96$\pm$0.05}}}    \\ \hline
\rowcolor[HTML]{E1E3F9} 
\cellcolor[HTML]{E1E3F9}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                        & 1.0                                    & 1.0                                                                 & 0.99                                  & 0.89                                                           & 1.0                                    & 0.933                                  \\  
\rowcolor[HTML]{E1E3F9} 
\cellcolor[HTML]{E1E3F9}                                                                                                    & COP-FT                                                                              & \textbf{0.0}                           & \textbf{0.0}                                                        & \textbf{0.0}                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.003                           \\ 
\rowcolor[HTML]{E1E3F9} 
\cellcolor[HTML]{E1E3F9}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & \textbf{0.0}                           & \textbf{0.0}                                                        & 0.005                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.008                           \\
\rowcolor[HTML]{E1E3F9} 
\multirow{-4}{*}{\cellcolor[HTML]{E1E3F9}\begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Rate \\ ($\downarrow$)\end{tabular}}             & \begin{tabular}[c]{@{}l@{}}\projectabbr\ (Ours)\end{tabular}                             & \textbf{0.0}                           & \textbf{0.0}                                                        & \textbf{0.0}                           & \textbf{0.0}                                                    & \textbf{0.0}                           & \textbf{0.0}                           \\ \hline
\rowcolor[HTML]{E1E3F9} 
\cellcolor[HTML]{E1E3F9}                                                                                                    & {\color[HTML]{000000} Guided DiffTime}                       & 23.21                                 & 16.35                                                              & 0.50                                  & 0.15                                                           & 1128.22                                & 5.23                                   \\  
\rowcolor[HTML]{E1E3F9} 
\cellcolor[HTML]{E1E3F9}                                                                                                    & COP-FT                                                                               & \textbf{0.0}                           & \textbf{0.0}                                                        & \textbf{0.0}                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.0002                           \\  
\rowcolor[HTML]{E1E3F9} 
\cellcolor[HTML]{E1E3F9}                                                                                                    & \begin{tabular}[c]{@{}l@{}}COP \end{tabular}                              & \textbf{0.0}                           & \textbf{0.0}                                                        & 0.0001                           & \textbf{0.0}                                                    & \textbf{0.0}                           & 0.0003                           \\  
\rowcolor[HTML]{E1E3F9} 
\multirow{-4}{*}{\cellcolor[HTML]{E1E3F9}\begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Magnitude\\ ($\downarrow$)\end{tabular}}        & \begin{tabular}[c]{@{}l@{}}\projectabbr\ (Ours)\end{tabular}                             & \textbf{0.0}                           & \textbf{0.0}                                                        &               \textbf{0.0}             & \textbf{0.0}                                                    & \textbf{0.0}                           &  \textbf{0.0}                          \\ \hline
\end{tabular}
\end{sc}
\end{small}
}
\end{center}
\caption{\textbf{\projectabbr\ outperforms existing baselines on sample quality and similarity metrics.} Yellow corresponds to sample quality metrics, and orange and violet correspond to similarity and constraint violation metrics, respectively. The best approach is shown in bold for each metric. Overall, we observe that \projectabbr\ maintains high sample quality (very low  FD and TSTR values) and the highest similarity with real time series samples (best values for the DTW and SSIM metrics). Our key intuition is that the adverse effects of the projection step are nullified by the subsequent denoising steps. Note that as the constraints are all convex, the COP variants and \projectabbr\ can achieve very low constraint violation.} 

\label{tab:main_results}
\end{table*}


% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

==> tables_latex/pdm_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!hbt]
% \centering
\scalebox{0.79}{
% \begin{tiny}
\begin{sc}
\rebuttal{
\begin{tabular}{lllllllll}
\hline
Dataset                                                                & Approach                                                & FTSD ($\downarrow$)           & TSTR   ($\downarrow$)                & DS   ($\downarrow$)                 & DTW    ($\downarrow$)             & SSIM      ($\uparrow$)          & \begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Rate\end{tabular} ($\downarrow$) & \begin{tabular}[c]{@{}l@{}}Constraint\\ Violation\\ Magnitude\end{tabular} ($\downarrow$) \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Air \\ Quality\end{tabular}} & PDM                                                  & 0.1503          & 0.205$\pm$0.005          & 0.254$\pm$0.014        & 2.544$\pm$1.96         & 0.342$\pm$0.148        & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \cline{2-9} 
                                                                        & \begin{tabular}[c]{@{}l@{}}CPS\\ (Ours)\end{tabular} & \textbf{0.0234} & \textbf{0.19$\pm$0.003}  & \textbf{0.06$\pm$0.01}   & \textbf{2.35$\pm$1.48} & \textbf{0.38$\pm$0.15} & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \hline
\multirow{2}{*}{Stocks}                                                 & PDM                                                  & 0.0368          & 0.044$\pm$0.001          & 0.0147$\pm$0.007         & 0.447$\pm$1.06         & 0.481$\pm$0.309        & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \cline{2-9} 
                                                                        & \begin{tabular}[c]{@{}l@{}}CPS\\ (Ours)\end{tabular} & \textbf{0.0023} & \textbf{0.041$\pm$0.001} & \textbf{0.006$\pm$0.004} & \textbf{0.20$\pm$0.71} & \textbf{0.73$\pm$0.26} & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \hline
\multirow{2}{*}{Traffic}                                                & PDM                                                  & 0.2714          & \textbf{0.29$\pm$0.008}  & 0.1313$\pm$0.053         & 3.547$\pm$1.34         & 0.249$\pm$0.192        & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \cline{2-9} 
                                                                        & \begin{tabular}[c]{@{}l@{}}CPS\\ (Ours)\end{tabular} & \textbf{0.2077} & \textbf{0.29$\pm$0.001}  & \textbf{0.02$\pm$0.01}   & \textbf{3.41$\pm$1.47} & \textbf{0.31$\pm$0.20} & \textbf{0.0}                                                          & \textbf{0.0}                                                               \\ \hline
\end{tabular}}
\end{sc}
% \end{tiny}
}
\caption{\rebuttal{\textbf{\projectabbr\ outperforms Projected Diffusion Models (PDM) on sample quality and similarity metrics.} On all the real-world datasets, we note that \projectabbr\ provides better sample quality metrics than PDM. The experimental setup is the same as in Table \ref{tab:main_results}. Both approaches provide perfect constraint satisfaction as we deal with linear and convex constraints. However, \projectabbr\ outperforms PDM in the Frechet Time Series Distance (FTSD), Train on Synthetic and Test on Real (TSTR), and the Discriminative Score (DS) metrics. Additionally, \projectabbr\ provides better similarity scores.}}
\label{tab:pdm_comp}
\end{table}
